Completeness of the ZX-calculus

The ZX-calculus is an intuitive but also mathematically strict graphical language for quantum computing, which is especially powerful for the framework of quantum circuits. Completeness of the ZX-calculus means any equality of matrices with size powers of $n$ can be derived purely diagrammatically. In this thesis, we give the first complete axiomatisation the ZX-calculus for the overall pure qubit quantum mechanics, via a translation from the completeness result of another graphical language for quantum computing -- the ZW-calculus. This paves the way for automated pictorial quantum computing, with the aid of some software like Quantomatic. Based on this universal completeness, we directly obtain a complete axiomatisation of the ZX-calculus for the Clifford+T quantum mechanics, which is approximatively universal for quantum computing, by restricting the ring of complex numbers to its subring corresponding to the Clifford+T fragment resting on the completeness theorem of the ZW-calculus for arbitrary commutative ring. Furthermore, we prove the completeness of the ZX-calculus (with just 9 rules) for 2-qubit Clifford+T circuits by verifying the complete set of 17 circuit relations in diagrammatic rewriting. In addition to completeness results within the qubit related formalism, we extend the completeness of the ZX-calculus for qubit stabilizer quantum mechanics to the qutrit stabilizer system. Finally, we show with some examples the application of the ZX-calculus to the proof of generalised supplementarity, the representation of entanglement classification and Toffoli gate, as well as equivalence-checking for the UMA gate.

==> Def_5.3.tex <==
\begin{proposition}(ZW rule $rei^x_2$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/reix2_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/reix2_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}~\newline
	\input{diagrams/reix2_proof.tikz}
\end{proof}
%\input{Def_5.3/reix2/prop_reix2}
\begin{proposition}(ZW rule $rei^x_3$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/reix3_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/reix3_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}~\newline
	\input{diagrams/reix3_proof.tikz}
\end{proof}
%\input{Def_5.3/reix3/prop_reix3}
\begin{proposition}\label{prop:natnx}(ZW rule $nat^\eta_x$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natnx_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natnx_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}~\newline
	\input{diagrams/natnx_proof.tikz}
\end{proof}
%\input{Def_5.3/natnx/prop_natnx}
\begin{proposition}(ZW rule $nat^\varepsilon_x$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natex_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natex_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Similar to proposition \ref{prop:natnx}.
\end{proof}
%\input{Def_5.3/natex/prop_natex}
\begin{proposition}\label{prop:reix1}(ZW rule $rei^x_1$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/reix1_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/reix1_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}~\newline
	\input{diagrams/reix1_proof.tikz}
\end{proof}
%\input{Def_5.3/reix1/prop_reix1}

==> Def_5.4.tex <==
\begin{proposition}(ZW rule $un^{co}_{w,L}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/uncowL_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/uncowL_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Similar proof in \cite{Emmanuel}, proposition 7 part $1b$. The rules used are $\ref{lem:inv}$, $S1$, $H2$, $H$, $S2$, $TR7$, $\ref{lem:hopf}$, $TR2$, $\ref{lem:3}$.
\end{proof}
%\input{Def_5.4/uncowL/prop_uncowL}
\begin{proposition}(ZW rule $un^{co}_{w,R}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/uncowR_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/uncowR_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $1b$. The rules used are $\ref{lem:inv}$, $S1$, $H2$, $H$, $S2$, $TR7$, $\ref{lem:hopf}$, $TR2$, $\ref{lem:3}$.
\end{proof}

%\input{Def_5.4/uncowR/prop_uncowR}
\begin{proposition}(ZW rule $nat^w_w$)~\newline\\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natww_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natww_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Claim:\\
	\input{diagrams/natww_claim.tikz}\\
	Proof of claim:\\
	$`\implies'$:\\
	\input{diagrams/natww_claimproof.tikz}\\
	$`\impliedby'$:\\
	\input{diagrams/natww_claimproof2.tikz}\\
	Hence we only have to prove\\
		$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natww_simon_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natww_simon_RHS.tikz}
	~\right\rrbracket_{WX}
	$
	\\
	which is proven in \cite{Emmanuel}, proposition 7 part $1a$. The rules used are $S1$, $B2$, $\ref{lem:4}$, $\ref{lem:5}$, $TR8$.
\end{proof}
%\input{Def_5.4/natww/prop_natww}
\begin{proposition}(ZW rule $nat^w_x$)~\newline\\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natwx_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natwx_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $7a$. The rules used are $H$, $\ref{lem:1}$, $S1$, $B2$.
\end{proof}
%\input{Def_5.4/natwx/prop_natwx}
\begin{proposition}(ZW rule $com^{co}_w$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/comcow_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/comcow_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}~\newline
	\input{diagrams/comcow_proof.tikz}\\
\end{proof}
%\input{Def_5.4/comcow/prop_comcow}
\begin{proposition}(ZW rule $nat^m_w$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natmw_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natmw_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7, part $5a$. It was proved in eight parts, (\textit{i}), (\textit{ii}), (\textit{iii}), (\textit{iv}), (\textit{v}), (\textit{vi}), (\textit{vii}), (\textit{viii}).
	
	The rules used in part (\textit{i}) are $B2$, $S1$, $H$, $TR5$, $\ref{lem:6b}$.
	
	The rules used in part (\textit{ii}) are $\ref{lem:4}$, $S1$, $B2$, $S1$, $TR11$, $\ref{lem:6b}$, $TR1$.
	
	The rules used in part (\textit{iii}) are $TR6$, $\ref{lem:4}$, $S1$, $TR8$, $\ref{lem:6b}$.
	
	The rules used in part (\textit{iv}) are $\ref{lem:4}$, $S1$, $B2$, $\ref{lem:6b}$, $TR11$.
	
	The rules used in part (\textit{v}) are $\ref{lem:6b}$, part (\textit{v}).
	
	The rules used in part (\textit{vi}) are part (\textit{i}), $\ref{lem:4}$, $TR9$, $S1$, $\ref{lem:6b}$, $\ref{lem:hopf}$, $TR1$, $K2$, part (\textit{iii}), part (\textit{v}), part (\textit{ii}).
	
	The rules used in part (\textit{vii}) are $\ref{lem:6b}$, $S1$, $TR1$, $B2$, $TR7$, $\ref{lem:4}$, $TR11$.
	
	The rules used in part (\textit{viii}) are $\ref{lem:6b}$, $H$, $B2$, $S1$, $\ref{lem:hopf}$, $\ref{lem:6}$.
	
	Finally, the proof of this proposition uses the rules $\ref{lem:4}$, $S1$, part (\textit{viii}), $\ref{lem:hopf}$, part (\textit{vii}), part (\textit{vi}), $B2$, $\ref{lem:com}$, $\ref{lem:7}$, $\ref{lem:6b}$, $TR1$.
\end{proof}
%\input{Def_5.4/natmw/prop_natmw}
\begin{proposition}(ZW rule $nat^{m \eta}_{w}$)~\newline\\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natmnw_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natmnw_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $5c$. The rules used are $\ref{lem:2}$, $B1$, $TR2$.
\end{proof}
%\input{Def_5.4/natmnw/prop_natmnw}
\begin{proposition}(ZW rule $nat^{m \eta}_{\varepsilon ,w}$)~\newline\\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natmnew_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natmnew_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part 5c. The rules used are $\ref{lem:2}$, $S1$, $B1$, $\ref{lem:inv}$.

\end{proof}
%\input{Def_5.4/natmnew/prop_natmnew}
\begin{proposition}(ZW rule $hopf$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/hopf_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/hopf_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $5d$. The rules used are $\ref{prop:rng-1}$, $\ref{lem:hopf}$, $S1$, $TR10$, $TR4$, $B1$.
\end{proof}
%\input{Def_5.4/hopf/prop_hopf}

==> Def_5.7.tex <==
\begin{proposition}(ZW rules $sym_{3,L}$ and $sym_{3,R}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/sym3_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/sym3_middle.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/sym3_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $0b$ and $0b'$ respectively. The rules used are $\ref{lem:4}$, $\ref{lem:com}$, $\ref{lem:6b}$, $S1$, $TR1$.
	%\input{Def_5.7/sym3/sym3_proof.tikz}
\end{proof}
%\input{Def_5.7/sym3/prop_sym3}
\begin{proposition}(ZW rule $sym_{2}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/sym2_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/sym2_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $0a$. The rules used are $S1$, $\ref{lem:com}$.
\end{proof}
%\input{Def_5.7/sym2/prop_sym2}
\begin{proposition}(ZW rule $inv$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/inv_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/inv_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $2a$. The rule used is $S1$.
\end{proof}
%\input{Def_5.7/inv/prop_inv}
\begin{proposition}(ZW rule $ant^\eta_x$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/antnx_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/antnx_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $7b$. The rules used are $\ref{lem:6b}$, $H$, $S1$.
\end{proof}
%\input{Def_5.7/antnx/prop_antnx}


==> Def_5.8.tex <==
\begin{proposition}(ZW rules $sym_{z,L}$ and $sym_{z,R}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/symz_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/symz_middle.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/symz_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof follows directly from rules $S1$ and $\ref{lem:com}$.
\end{proof}
%\input{Def_5.8/symz/prop_symz}
\begin{proposition}(ZW rule $un^{co}_{z,R}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/uncozR_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/uncozR_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof follows directly from rule $S1$.
\end{proof}
%\input{Def_5.8/uncozR/prop_uncozR}
\begin{proposition}(ZW rule $nat^z_z$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natzz_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natzz_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof follows directly from rules $S1$ and $\ref{lem:com}$.
\end{proof}
%\input{Def_5.8/natzz/prop_natzz}
\begin{proposition}\label{prop:ph}(ZW rule $ph$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/ph_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/ph_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}~\newline
	\input{diagrams/ph_proof.tikz}.
\end{proof}
%\input{Def_5.8/ph/prop_ph}
\begin{proposition}(ZW rule $nat^m_c$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natnc_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natnc_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $3a$. The rule used is $\ref{lem:6b}$.
\end{proof}
%\input{Def_5.8/natnc/prop_natnc}
\begin{proposition}(ZW rule $nat^m_c$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natmc_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natmc_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $6a$. The rules used are $S1$, $B2$, $TR10$.
\end{proof}
%\input{Def_5.8/natmc/prop_natmc}
\begin{proposition}(ZW rule $loop$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/loop_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/loop_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $6c$. The rules used are $\ref{lem:hopf}$, $B1$, $TR2$.
\end{proof}
%\input{Def_5.8/loop/prop_loop}
\begin{proposition}(ZW rule $unx$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/unx_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/unx_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof in \cite{Emmanuel}, proposition 7 part $X$. The rules used are $\ref{lem:1}$, $S1$, $B2$, $\ref{lem:6}$, $TR5$.
\end{proof}
%\input{Def_5.8/unx/prop_unx}

==> Def_5.9.tex <==
\begin{proposition}(ZW rule $rng_1$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/rng1_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/rng1_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof follows directly from rule $L3$.
\end{proof}
%\input{Def_5.9/rng1/prop_rng1}
\begin{proposition}\label{prop:rng-1}(ZW rule $rng_{-1}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/rng-1_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/rng-1_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Similar to \ref{prop:ph}.
\end{proof}
%\input{Def_5.9/rng-1/prop_rng-1}
\begin{proposition}(ZW rule $rng^{r,s}_{\times}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/rngrsx_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/rngrsx_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof follows directly from rules $S1$, $L4$, $L5$.
\end{proof}
%\input{Def_5.9/rngrsx/prop_rngrsx}
\begin{proposition}(ZW rule $rng^{r,s}_{+}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/rngrsp_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/rngrsp_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof follows directly from rule $AD$.
\end{proof}
%\input{Def_5.9/rngrsp/prop_rngrsp}
\begin{proposition}(ZW rule $nat^{r}_{c}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natrc_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natrc_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof follows directly from rules $TR13$, $TR14$.
\end{proof}
%\input{Def_5.9/natrc/prop_natrc}
\begin{proposition}(ZW rule $nat^{r}_{\varepsilon c}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/natrec_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/natrec_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof follows directly from rules $\ref{lem:S4}$, $L2$.
\end{proof}
%\input{Def_5.9/natrec/prop_natrec}
\begin{proposition}(ZW rule $ph^{r}$)~\newline \\
	$
	ZX\vdash
	\left\llbracket~
	\input{diagrams/phr_LHS.tikz}
	~\right\rrbracket_{WX}
	=
	\left\llbracket~
	\input{diagrams/phr_RHS.tikz}
	~\right\rrbracket_{WX}
	$
\end{proposition}

\begin{proof}
	Proof follows directly from rules $S1$, $L1$.
\end{proof}
%\input{Def_5.9/phr/prop_phr}

==> Lemmas.tex <==
\begin{lemma}~\newline
	\label{lem:6b}
	$
	\input{diagrams/lemma6b.tikz}
	$
\end{lemma}

\begin{proof}
	Proof in \cite{bpw}. The rules used are $S1$, $S2$, $S3$, $H$, $H2$, $H3$, $B1$, $B2$, $EU$, $\ref{lem:inv}$.
\end{proof}

\begin{lemma}~\newline
	\label{lem:hopf}
	$
	\input{diagrams/lemmahopf.tikz}
	$
\end{lemma}

\begin{proof}
	Proof in \cite{bpw}. The rules used are $S1$, $S2$, $S3$, $H2$, $H3$, $H$, $B1$, $B2$.
\end{proof}

\begin{lemma}~\newline
	\label{lem:com}
	$
	\input{diagrams/lemmacom.tikz}
	$
\end{lemma}

\begin{proof}
	Proof in \cite{bpw}. The rules used are \ref{lem:hopf}, $B2$, $S2$, $H2$, $S1$, $H$, $B1$.
\end{proof}

\begin{lemma}~\newline
	\label{lem:inv}
	$
	\input{diagrams/lemmainv.tikz}
	$
\end{lemma}

\begin{proof}~\newline
	\input{diagrams/lemmainv_proof.tikz}
\end{proof}

\begin{lemma}~\newline
	\label{lem:S4}
	$
	\tikzfig{diagrams//alphadelete}
	$
\end{lemma}

\begin{proof}
	Proof in \cite{bpw}. The rules used are $S1$, $B1$, $K2$, $\ref{lem:6b}$, $\ref{lem:inv}$.
\end{proof}

\begin{lemma}~\newline
	\label{lem:1}
	$
	\input{diagrams/lemma1.tikz}
	$
\end{lemma}

\begin{proof}~\newline
	\input{diagrams/lemma1_proof.tikz}
\end{proof}

\begin{lemma}~\newline
	\label{lem:2}
	$
	\input{diagrams/lemma2.tikz}
	$
\end{lemma}

\begin{proof}
	Proof in \cite{Emmanuel} lemma $33$. The rules used are \ref{lem:hopf}, \ref{lem:inv}, $B1$, $TR2$.
\end{proof}

\begin{lemma}~\newline
	\label{lem:3}
	$
	\input{diagrams/lemma3.tikz}
	$
\end{lemma}

\begin{proof}
	Proof in \cite{Emmanuel} lemma $19$. The rules used are \ref{lem:hopf}, \ref{lem:inv}, $B1$, $TR2$.
\end{proof}

\begin{lemma}~\newline
	\label{lem:4}
	$
	\input{diagrams/lemma4.tikz}
	$
\end{lemma}

\begin{proof}
	Proof in \cite{Emmanuel} lemma $26$. The rules used are $B2, S1, TR7$.
\end{proof}

\begin{lemma}~\newline
	\label{lem:5}
	$
	\input{diagrams/lemma5.tikz}
	$
\end{lemma}

\begin{proof}
	Straightforward application of rules $\ref{lem:com}$ and $TR8$.
\end{proof}

\begin{lemma}~\newline
	\label{lem:6}
	$
	\input{diagrams/lemma6.tikz}
	$
	\\
	Equivalently,\\
	$
	\input{diagrams/lemma6v2.tikz}
	$
\end{lemma}

\begin{proof}
	Straightforward application of rules $H$ and $EU$.
\end{proof}

\begin{lemma}~\newline
	\label{lem:7}
	$
	\input{diagrams/lemma7.tikz}
	$
\end{lemma}

\begin{proof}~\newline
	$
	\input{diagrams/lemma7_proof.tikz}
	$
\end{proof}


%%%%%%%%


==> Minimal_ZX_LMCS/defs.tex <==
\newcommand{\TODO}[1]{%
\typeout{WARNING!!! there is still a TODO left}
\marginpar{\textbf{!TODO: }\emph{#1}}
}

\newcommand{\denoteb}[1]{% --``semantic'' brakets
\left\llbracket #1 \right\rrbracket} 

\newcommand{\den}[1]{\denoteb{#1}^\natural}


\def\alpvec{[\vec{\alpha}]}
\def\alpprevec{\vec{\alpha}}
\def\betvec{[\vec{\beta}_j]}
\def\betprevec{\vec{\beta}_j}

\def\blackmu{\mu_{\smallblackdot}} 
\def\graymu {\mu_{\smallgraydot}}
\def\whitemu{\mu_{\smallwhitedot}}

\def\blacketa{\eta_{\smallblackdot}} 
\def\grayeta {\eta_{\smallgraydot}}
\def\whiteeta{\eta_{\smallwhitedot}}

\def\blackdelta{\delta_{\smallblackdot}} 
\def\graydelta {\delta_{\smallgraydot}}
\def\whitedelta{\delta_{\smallwhitedot}}

\def\blackepsilon{\epsilon_{\smallblackdot}} 
\def\grayepsilon {\epsilon_{\smallgraydot}}
\def\whiteepsilon{\epsilon_{\smallwhitedot}}

% \def\whiteeta{\eta_{\!\smallwhitedot}}
% \def\whitevarepsilon{\varepsilon_{\!\smallwhitedot}}

\def\whitePhi{\Phi_{\!\smallwhitedot}}
\def\graymeas{m_{\!\smallgraydot}}

\newcommand{\Owg}{\ensuremath{{\cal O}_{\!\smallwhitedot\!,\!\smallgraydot}}}
\newcommand{\whiteK}{\ensuremath{{\cal  K}_{\!\smallwhitedot}}}
\newcommand{\grayK}{\ensuremath{{\cal  K}_{\!\smallgraydot}}}


% BRAS AND KETS
\newcommand{\bra}[1]{\ensuremath{\left\langle #1 \right|}}
\newcommand{\ket}[1]{\ensuremath{\left|  #1 \right\rangle}}
\newcommand{\roundket}[1]{\ensuremath{\left|  #1 \right)}}
\newcommand{\braket}[2]{\ensuremath{\langle#1|#2\rangle}}
\newcommand{\ketbra}[2]{\ensuremath{\ket{#1}\!\bra{#2}}}

\newcommand{\innp}[2]{\braket{#1}{#2}}
\newcommand{\outp}[2]{\ketbra{#1}{#2}}

\newcommand{\ketGHZ} {\ket{\textit{GHZ}\,}}
\newcommand{\ketW}   {\ket{\textit{W\,}}}
\newcommand{\ketBell}{\ket{\textit{Bell\,}}}
\newcommand{\ketEPR} {\ket{\textit{EPR\,}}}
\newcommand{\ketGHZD}{\ket{\textrm{GHZ}^{(D)}}}
\newcommand{\ketWD}  {\ket{\textrm{W}^{(D)}}}

\newcommand{\braGHZ} {\bra{\textit{GHZ}\,}}
\newcommand{\braW}   {\bra{\textit{W\,}}}
\newcommand{\braBell}{\bra{\textit{Bell\,}}}
\newcommand{\braEPR} {\bra{\textit{EPR\,}}}

\newcommand{\CX}{\wedge X}
\newcommand{\CZ}{\wedge Z}

%%%% useful cats notation
\newcommand{\id}[1]{\ensuremath{1_{#1}}}

\newcommand{\rw}{\Rightarrow}
\newcommand{\RW}[1]{\stackrel{#1}{\Rightarrow}}
\newcommand{\EQ}[1]{\stackrel{#1}{=}}

\newcommand{\denote}[1]{% --``semantic'' brakets
\llbracket #1 \rrbracket} 

%%%%SIMON DIAG
\newcommand{\dH}{\tikzfig{scalars-s//Had4}}
\newcommand{\sdH}{\tikzfig{scalars-s//Had5}}
\newcommand{\dempty}{\tikzfig{scalars-s//emptysquare-small}}
\newcommand{\dsigma}{\tikzfig{scalars-s//swap}}
\newcommand{\ldsigma}{\tikzfig{scalars-s//swap-large}}
\newcommand{\dcup}{\tikzfig{scalars-s//cup}}
\newcommand{\drcup}{\raisebox{-0.15cm}{\tikzfig{scalars-s//cup}}}
\newcommand{\drcap}{\raisebox{0.15cm}{\tikzfig{scalars-s//cap}}}
%\newcommand{\ldrcup}{\raisebox{-0.15cm}{\tikzfig{scalars//cup-large}}}
%\newcommand{\ldrcap}{\raisebox{0.15cm}{\tikzfig{scalars//cap-large}}}

\newcommand{\dsigmaf}{\tikzfig{scalars-s//swapf}}
\newcommand{\dHf}{\tikzfig{scalars-s//Had4f}}
\newcommand{\drcupf}{\raisebox{-0.15cm}{\tikzfig{scalars-s//cupf}}}
\newcommand{\drcapf}{\raisebox{0.15cm}{\tikzfig{scalars-s//capf}}}

\newcommand{\dgd}{\!\tikzfig{scalars-s//sspiderg}\!}
\newcommand{\drd}{\!\tikzfig{scalars-s//sspiderr}\!}
\newcommand{\droot}{\raisebox{-0.1cm}{\tikzfig{scalars-s//1line}}}
\newcommand{\diroot}{\raisebox{-0.1cm}{\tikzfig{scalars-s//iroot}}}


\newcommand{\dcap}{\tikzfig{scalars-s//cap}}
\newcommand{\did}{\tikzfig{scalars-s//Id}}
\newcommand{\didf}{\tikzfig{scalars-s//Idf}}

\newcommand{\gdzz}{\tikzfig{scalars-s//RZ00alpha}}
\newcommand{\gdzo}{\tikzfig{scalars-s//RZ01alpha}}
\newcommand{\gdzopi}{\tikzfig{scalars-s//RZ01pi}}
\newcommand{\gdzoz}{\tikzfig{scalars-s//RZ01z}}
\newcommand{\gdoo}{\tikzfig{scalars-s//RZ11alpha}}
\newcommand{\gdto}{\tikzfig{scalars-s//RZ21alpha}}
\newcommand{\gpi}{\tikzfig{scalars-s//RZ00pi}}
\newcommand{\rpi}{\tikzfig{scalars-s//RZ00pir}}

\newcommand{\gdot}{\tikzfig{scalars-s//RZ00zero}}

\newcommand{\rdzz}{\tikzfig{scalars-s//RX00alpha}}
\newcommand{\rdzo}{\tikzfig{scalars-s//RX01alpha}}
\newcommand{\rdoo}{\tikzfig{scalars-s//RX11alpha}}
\newcommand{\rdto}{\tikzfig{scalars-s//RX21alpha}}


%%%%


%%%%% nicely fornatted names for categories

\newcommand{\catname}[1]{\ensuremath{\mathbf{#1}}\xspace}
\newcommand{\catnamesub}[2]{\ensuremath{\mathbf{#1}_{#2}}\xspace}
\newcommand{\catnamesup}[2]{\ensuremath{\mathbf{#1}^{#2}}\xspace}


\newcommand{\spek}{\catname{Spek}}
\newcommand{\stab}{\catname{Stab}}
\newcommand{\qubit}{\catname{Qubit}}
\newcommand{\fhilb}{\catname{FHilb}}
\newcommand{\fhilbd}{\catnamesub{FHilb}{D}}
\newcommand{\fhilbii}{\catnamesub{FHilb}{2}}
\newcommand{\fdhilb}{\fhilb}
\newcommand{\fdhilbd}{\fhilbd}
\newcommand{\fdhilbii}{\fhilbii}
\newcommand{\frel}{\catname{FRel}}
\newcommand{\FRel}{\frel}
\newcommand{\Frel}{\frel}
\newcommand{\freld}{\catnamesub{FRel}{D}}
\newcommand{\Freld}{\freld}
\newcommand{\FRelD}{\freld}
\newcommand{\frelii}{\catnamesub{FRel}{2}}
\newcommand{\Frelii}{\frelii}
\newcommand{\FRelii}{\frelii}
\newcommand{\fset}{\catname{FSet}}
\newcommand{\perm}{\catname{Perm}}
\newcommand{\stoch}{\catname{Stoch}}
\newcommand{\bool}{\catname{Bool}}
\newcommand{\symgrp}{\catname{SymGrp}}

\newcommand{\boolcircs}{\catname{BoolCirc}}
\newcommand{\boolcirc}{\boolcircs}
\newcommand{\qcircs}{\catname{QuCirc}}
\newcommand{\qcirc}{\qcircs}

\newcommand{\CC}{\catname{C}}
\newcommand{\CCop}{\catnamesup{C}{\mathrm{op}}}
\newcommand{\DD}{\catname{D}}
\newcommand{\DDop}{\catnamesup{D}{\mathrm{op}}}

% CATEGORY VARIABLES
\newcommand{\catC}{\CC}   %{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\catCop}{\CCop}   %{\ensuremath{\mathcal{C}^{\mathrm{op}}}\xspace}
\newcommand{\catD}{\DD}    %{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\catDop}{\DDop}   %{\ensuremath{\mathcal{D}^{\mathrm{op}}}\xspace}


% STANDARD CATEGORIES
% \newcommand{\catSet}{\ensuremath{\textrm{\bf Set}}\xspace}
% \newcommand{\catRel}{\ensuremath{\textrm{\bf Rel}}\xspace}
\newcommand{\catFRel}{\frel}  % {\ensuremath{\textrm{\bf FRel}}\xspace}
% \newcommand{\catVect}{\ensuremath{\textrm{\bf Vect}}\xspace}
% \newcommand{\catFVect}{\ensuremath{\textrm{\bf FVect}}\xspace}
\newcommand{\catFHilb}{\fhilb}  %  {\ensuremath{\textrm{\bf FHilb}}\xspace}
% \newcommand{\catHilb}{\ensuremath{\textrm{\bf Hilb}}\xspace}
% \newcommand{\catSuperHilb}{\ensuremath{\textrm{\bf SuperHilb}}\xspace}
% \newcommand{\catAb}{\ensuremath{\textrm{\bf Ab}}\xspace}
% \newcommand{\catTop}{\ensuremath{\textrm{\bf Top}}\xspace}
% \newcommand{\catCHaus}{\ensuremath{\textrm{\bf CHaus}}\xspace}
% \newcommand{\catHaus}{\ensuremath{\textrm{\bf Haus}}\xspace}
% \newcommand{\catGraph}{\ensuremath{\textrm{\bf Graph}}\xspace}
% \newcommand{\catMat}{\ensuremath{\textrm{\bf Mat}}\xspace}
% \newcommand{\catGr}{\ensuremath{\textrm{\bf Gr}}\xspace}
\newcommand{\catSpek}{\spek}  %{\ensuremath{\textrm{\bf Spek}}\xspace}

%\DeclareMathOperator{\CP}{CP}

%%%%%%%%%% Stolen from Aleks's Quantum Computation notes

\newcommand{\boxmap}[1]{\,\tikz[dotpic]{\node[style=square box] (x) {$#1$};\draw(0,-1)--(x)--(0,1);}\,}

\newcommand{\map}[1]{\,\tikz[dotpic]{\node[style=map] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\mapdag}[1]{\,\tikz[dotpic]{\node[style=mapdag] (x) {$#1$};\draw(0,-1.3)--(x)--(0,1.3);}\,}

\newcommand{\pointmap}[1]{\,\tikz[dotpic]{\node[style=point] (x) at (0,-0.5) {$#1$};\draw (x)--(0,1);}\,}

\newcommand{\copointmap}[1]{\,\tikz[dotpic]{\node[style=copoint] (x) at (0,0.5) {$#1$};\draw (x)--(0,-1);}\,}

\newcommand{\graypointmap}[1]{\,\tikz[dotpic]{\node[style=gray point] (x) at (0,-0.5) {$#1$};\draw (x)--(0,1);}\,}



% ========================
% = COMMUTATIVE DIAGRAMS =
% ========================

\tikzstyle{cdiag}=[matrix of math nodes, row sep=3em, column sep=3em, text height=1.5ex, text depth=0.25ex,inner sep=0.5em]
\tikzstyle{arrow above}=[transform canvas={yshift=0.5ex}]
\tikzstyle{arrow below}=[transform canvas={yshift=-0.5ex}]

\newcommand{\csquare}[8]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2);
\end{tikzpicture}
}

% commands for putting pushout/pullback brackets on commutative diags
\newcommand{\NWbracket}[1]{%
\draw #1 +(-0.25,0.5) -- +(-0.5,0.5) -- +(-0.5,0.25);}
\newcommand{\NEbracket}[1]{%
\draw #1 +(0.25,0.5) -- +(0.5,0.5) -- +(0.5,0.25);}
\newcommand{\SWbracket}[1]{%
\draw #1 +(-0.25,-0.5) -- +(-0.5,-0.5) -- +(-0.5,-0.25);}
\newcommand{\SEbracket}[1]{%
\draw #1 +(0.25,-0.5) -- +(0.5,-0.5) -- +(0.5,-0.25);}
\newcommand{\THETAbracket}[2]{%
\draw [rotate=#1] #2 +(0.25,0.5) -- +(0.5,0.5) -- +(0.5,0.25);}

\newcommand{\posquare}[8]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node [swap] {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2);
    \NWbracket{(m-2-2)}
\end{tikzpicture}
}

\newcommand{\pbsquare}[8]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node [swap] {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2);
  \SEbracket{(m-1-1)}
\end{tikzpicture}
}

\newcommand{\ctri}[6]{
    \begin{tikzpicture}[-latex]
        \matrix (m) [cdiag,ampersand replacement=\&] { #1 \& #2 \\ #3 \& \\ };
        \path [arrs] (m-1-1) edge node {$#4$} (m-1-2)
              (m-1-1) edge node [swap] {$#5$} (m-2-1)
              (m-2-1) edge node [swap] {$#6$} (m-1-2);
    \end{tikzpicture}
}

\newcommand{\crun}[5]{
\ensuremath{#1 \overset{#2}{\longrightarrow} #3 \overset{#4}{\longrightarrow} #5}
}

\newcommand{\cspan}[5]{
\ensuremath{#1 \overset{#2}{\longleftarrow} #3
               \overset{#4}{\longrightarrow} #5}
}

\newcommand{\ccospan}[5]{
\ensuremath{#1 \overset{#2}{\longrightarrow} #3
               \overset{#4}{\longleftarrow} #5}
}

\newcommand{\cpair}[4]{
\begin{tikzpicture}
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\};
    \path [arrs] (m-1-1.20) edge node {$#3$} (m-1-2.160)
                 (m-1-1.-20) edge node [swap] {$#4$} (m-1-2.-160);
\end{tikzpicture}
}

\newcommand{\csquareslant}[9]{
\begin{tikzpicture}[-latex]
    \matrix(m)[cdiag,ampersand replacement=\&]{
    #1 \& #2 \\
    #3 \& #4  \\};
    \path [arrs] (m-1-1) edge node {$#5$} (m-1-2)
                 (m-2-1) edge node {$#6$} (m-2-2)
                 (m-1-1) edge node [swap] {$#7$} (m-2-1)
                 (m-1-2) edge node {$#8$} (m-2-2)
                 (m-1-2) edge node [swap] {$#9$} (m-2-1);
\end{tikzpicture}
}


\newcommand{\zxcalculus}{\textsc{zx}-calculus\xspace}
\newcommand{\iso}{\ensuremath{\cong}}


\newcommand{\zxs}{\textup{ZX}_{\textsf{simp}}}
\newcommand{\zxo}{\textup{ZX}_{\textsf{orig}}}
\newcommand{\zxc}{\textup{ZX}_{\textsf{ccc}}}
\newcommand{\zxb}{\textup{ZX}_{\textsf{bac}}}

\newcommand{\ct}{{\quad\rightarrow\quad}}


%% Miriam's definitions
\newcommand{\NOT}{\textsc{not}}
\newcommand{\ZX}{\textsc{zx}}
\newcommand{\intf}[1]{\ensuremath{\left\llbracket #1 \right\rrbracket}} % interpretation functor
\let\oldt=\t % rename builtin command \t{}
\renewcommand{\t}[1]{\ensuremath{^{\otimes #1}}} % tensor power
\tikzstyle{bscalar}=[star,fill=black,draw=black,minimum size=8pt,inner sep=0pt]
%% Miriam's definitions end

%% Harny's definitions
\tikzstyle{emptynode}=[circle,fill=none,draw=none,inner sep=1.5pt]
%% Harny's definitions end



==> Minimal_ZX_LMCS/tikzfigures.tex <==
% define in-prose representations for lots of generators

%%%%REVERSED BY BOB %%%%%%%%

\newcommand{\dotcounit}[1]{%
\,\begin{tikzpicture}[dotpic,yshift=-1mm]
\node [#1] (a) at (0,0.25) {}; 
\draw [medium diredge] (0,-0.2)--(a);
\end{tikzpicture}\,}
\newcommand{\dotunit}[1]{%
\,\begin{tikzpicture}[dotpic,yshift=1.5mm]
\node [#1] (a) at (0,-0.25) {}; 
\draw [medium diredge] (a)--(0,0.2);
\end{tikzpicture}\,}
\newcommand{\dotcomult}[1]{%
\,\begin{tikzpicture}[dotpic,yshift=0.5mm]
	\node [#1] (a) {};
	\draw [medium diredge] (-90:0.55)--(a);
	\draw [medium diredge] (a) -- (45:0.6);
	\draw [medium diredge] (a) -- (135:0.6);
\end{tikzpicture}\,}
\newcommand{\dotmult}[1]{%
\,\begin{tikzpicture}[dotpic]
	\node [#1] (a) {};
	\draw [medium diredge] (a) -- (90:0.55);
	\draw [medium diredge] (a) (-45:0.6) -- (a);
	\draw [medium diredge] (a) (-135:0.6) -- (a);
\end{tikzpicture}\,}

%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dotidualiser}[1]{%
\begin{tikzpicture}[dotpic,yshift=1.5mm]
	\node [#1] (a) {};
	\draw [medium diredge] (a) to (-90:0.35);
	\draw [medium diredge] (a) to (90:0.35);
\end{tikzpicture}}
\newcommand{\dotdualiser}[1]{%
\begin{tikzpicture}[dotpic,yshift=1.5mm]
	\node [#1] (a) {};
	\draw [medium diredge] (-90:0.35) to (a);
	\draw [medium diredge] (90:0.35) to (a);
\end{tikzpicture}}
\newcommand{\dottickunit}[1]{%
\begin{tikzpicture}[dotpic,yshift=-1mm]
\node [#1] (a) at (0,0.35) {}; 
\draw [postaction=decorate,
       decoration={markings, mark=at position 0.3 with \edgetick},
       decoration={markings, mark=at position 0.85 with \edgearrow}] (a)--(0,-0.25);
\end{tikzpicture}}
\newcommand{\dottickcounit}[1]{%
\begin{tikzpicture}[dotpic,yshift=1mm]
\node [#1] (a) at (0,-0.35) {}; 
\draw [postaction=decorate,
       decoration={markings, mark=at position 0.8 with \edgetick},
       decoration={markings, mark=at position 0.45 with \edgearrow}] (0,0.25) -- (a);
\end{tikzpicture}}
\newcommand{\dotonly}[1]{%
\,\begin{tikzpicture}[dotpic,yshift=-0.3mm]
\node [#1] (a) at (0,0) {};
\end{tikzpicture}\,}
%NEW:
\newcommand{\smalldotonly}[1]{%
\,\begin{tikzpicture}[dotpic,yshift=-0.15mm]
\node [#1] (a) at (0,0) {};
\end{tikzpicture}\,}
%
\newcommand{\dotthreestate}[1]{%
\,\begin{tikzpicture}[dotpic,yshift=2.5mm]
	\node [#1] (a) at (0,0) {};
	\draw (a) -- (0,-0.6);
	\draw [bend right] (a) to (-0.4,-0.6) (0.4,-0.6) to (a);
\end{tikzpicture}\,}
\newcommand{\dotcap}[1]{%
\,\begin{tikzpicture}[dotpic,yshift=2.5mm]
	\node [#1] (a) at (0,0) {};
	\draw [bend right,medium diredge] (a) to (-0.4,-0.6);
	\draw [bend left,medium diredge] (a) to (0.4,-0.6);
\end{tikzpicture}\,}
\newcommand{\dotcup}[1]{%
\,\begin{tikzpicture}[dotpic,yshift=4mm]
	\node [#1] (a) at (0,-0.6) {};
	\draw [bend right,medium diredge] (-0.4,0) to (a);
	\draw [bend left,medium diredge] (0.4,0) to (a);
\end{tikzpicture}\,}

% this doesn't have a colour
\newcommand{\tick}{%
\,\,\begin{tikzpicture}[dotpic]
	\node [style=none] (a) at (0,0.35) {};
	\node [style=none] (b) at (0,-0.35) {};
	\draw [dirtickedge] (a) -- (b);
\end{tikzpicture}\,\,}

% these only make sense in black
\newcommand{\lolli}{%
\,\begin{tikzpicture}[dotpic,yshift=-1mm]
	\path [use as bounding box] (-0.25,-0.25) rectangle (0.25,0.5);
	\node [style=dot] (a) at (0, 0.15) {};
	\node [style=none] (b) at (0, -0.25) {};
	\draw [medium diredge] (a) to (b.center);
	\draw [diredge, out=45, looseness=1.00, in=135, loop] (a) to ();
\end{tikzpicture}\,}

\newcommand{\cololli}{%
\,\begin{tikzpicture}[dotpic]
	\path [use as bounding box] (-0.25,-0.5) rectangle (0.25,0.5);
	\node [style=none] (a) at (0, 0.5) {};
	\node [style=dot] (b) at (0, 0) {};
	\draw [diredge, in=-45, looseness=2.00, out=-135, loop] (b) to ();
	\draw [medium diredge] (a.center) to (b);
\end{tikzpicture}\,}

% BLACK DOTS
\newcommand{\blackdot}{\dotonly{dot}}
\newcommand{\smallblackdot}{\smalldotonly{smalldot}}%NEW
\newcommand{\unit}{\dotunit{dot}}
\newcommand{\counit}{\dotcounit{dot}}
\newcommand{\mult}{\dotmult{dot}}
\newcommand{\comult}{\dotcomult{dot}}
\newcommand{\tickunit}{\dottickunit{dot}}
\newcommand{\tickcounit}{\dottickcounit{dot}}
\newcommand{\dualiser}{\dotdualiser{dot}}
\newcommand{\idualiser}{\dotidualiser{dot}}
\newcommand{\threestate}{\dotthreestate{dot}}
\newcommand{\blackcap}{\dotcap{dot}}
\newcommand{\blackcup}{\dotcup{dot}}

\newcommand{\blackobs}{\ensuremath{\mathcal O_{\!\smallblackdot}}\xspace}

% WHITE DOTS
\newcommand{\whitedot}{\dotonly{white dot}}
\newcommand{\smallwhitedot}{\smalldotonly{smallwhitedot}}%NEW
\newcommand{\whiteunit}{\dotunit{white dot}}
\newcommand{\whitecounit}{\dotcounit{white dot}}
\newcommand{\whitemult}{\dotmult{white dot}}
\newcommand{\whitecomult}{\dotcomult{white dot}}
\newcommand{\whitetickunit}{\dottickunit{white dot}}
\newcommand{\whitetickcounit}{\dottickcounit{white dot}}
\newcommand{\whitecap}{\dotcap{white dot}}
\newcommand{\whitecup}{\dotcup{white dot}}


\newcommand{\whiteobs}{\ensuremath{\mathcal O_{\!\smallwhitedot}}\xspace}


% ALTERNATE WHITE DOTS
\newcommand{\altwhitedot}{\dotonly{alt white dot}}
\newcommand{\altwhiteunit}{\dotunit{alt white dot}}
\newcommand{\altwhitecounit}{\dotcounit{alt white dot}}
\newcommand{\altwhitemult}{\dotmult{alt white dot}}
\newcommand{\altwhitecomult}{\dotcomult{alt white dot}}
\newcommand{\altwhitetickunit}{\dottickunit{alt white dot}}
\newcommand{\altwhitetickcounit}{\dottickcounit{alt white dot}}
\newcommand{\altwhitecap}{\dotcap{alt white dot}}
\newcommand{\altwhitecup}{\dotcup{alt white dot}}

% GRAY DOTS
\newcommand{\graydot}{\dotonly{gray dot}}
\newcommand{\smallgraydot}{\smalldotonly{smallgraydot}}%NEW
%\newcommand{\graysmalldot}{\smalldotonly{gray dot}}
\newcommand{\grayunit}{\dotunit{gray dot}}
\newcommand{\graycounit}{\dotcounit{gray dot}}
\newcommand{\graymult}{\dotmult{gray dot}}
\newcommand{\graycomult}{\dotcomult{gray dot}}
\newcommand{\graytickunit}{\dottickunit{gray dot}}
\newcommand{\graytickcounit}{\dottickcounit{gray dot}}
\newcommand{\graycap}{\dotcap{gray dot}}
\newcommand{\graycup}{\dotcup{gray dot}}

\newcommand{\grayobs}{\ensuremath{\mathcal O_{\!\smallgraydot}}\xspace}


\newcommand{\blacktranspose}{\ensuremath{{\,\blackdot\!\textrm{\rm\,T}}}}
\newcommand{\whitetranspose}{\ensuremath{{\!\!\altwhitedot\!\!}}}
\newcommand{\graytranspose}{\ensuremath{{\,\graydot\!\textrm{\rm\,T}}}}

\newcommand{\whiteconjugate}{\ensuremath{{\!\!\altwhitedot\!\!}}}

% \newcommand{\spider}[4][dot]{\node [#1] (#2) at (0,0) {};
% \node [bn] (#2_d1) at (-1,1) {};
% \node [bn] (#2_d2) at (-0.5,1) {};
% \node [bn] (#2_dm) at (1,1) {};
% \node [bn] (#2_c1) at (-1,-1) {};
% \node [bn] (#2_c2) at (-0.5,-1) {};
% \node [bn] (#2_cn) at (1,-1) {};

% \node [anchor=west] at (#2_dm.east) {$#3$};
% \node [anchor=west] at (#2_cn.east) {$#4$};
% \node at (0.2,0.7) {\small{...}};
% \node at (0.2,-0.7) {\small{...}};

% \draw (#2)--(#2_d1) (#2)--(#2_d2) (#2)--(#2_dm);
% \draw (#2)--(#2_c1) (#2)--(#2_c2) (#2)--(#2_cn);}

\newcommand{\circl}{\begin{tikzpicture}[dotpic]
		\node [style=none] (a) at (-0.25, 0.25) {};
		\node [style=none] (b) at (0.25, 0.25) {};
		\node [style=none] (c) at (-0.25, -0.25) {};
		\node [style=none] (d) at (0.25, -0.25) {};
		\draw [in=45, out=135] (b.center) to (a.center);
		\draw [in=135, out=225] (a.center) to (c.center);
		\draw [in=225, out=-45] (c.center) to (d.center);
		\draw [style=diredge, in=-45, out=45] (d.center) to (b.center);
\end{tikzpicture}}

% \newcommand{\icircl}{\begin{tikzpicture}[dotpic]
% 	\node [circle,draw=black,inner sep=1pt] {\footnotesize\sf{}{$-$}};
% \end{tikzpicture}}

% \newcommand{\rtcircl}{\ensuremath{\sqrt{\begin{tikzpicture}[dotpic]
% 	\node [circle,draw=black,inner sep=1pt] {\tiny\sf\phantom{$-$}};
% \end{tikzpicture}}}}
% \newcommand{\rticircl}{\ensuremath{\sqrt{\begin{tikzpicture}[dotpic]
% 	\node [circle,draw=black,inner sep=1pt] {\tiny\bf\sf{}{$-$}};
% \end{tikzpicture}}}}

% \newcommand{\dcircl}{\begin{tikzpicture}[dotpic]
% 	\draw [use as bounding box,draw=none] (-0.15,-0.3) rectangle (0.15,0.3);
% 	\node [small dot] (0) {};
% 	\draw [uploop] (0) to ();
% 	\draw [downloop] (0) to ();
% \end{tikzpicture}}


==> Minimal_ZX_LMCS/tikzstyles.tex <==
%MY GROUND:
\tikzstyle{env}=[copoint,regular polygon rotate=0,minimum width=0.2cm, fill=black]

%\definecolor{green}{rgb}{1,0.2,0.3}
%SIMON'S GROUND:
%
%\newcommand{\ground}[2]{
%\node[inner sep=0mm] (#1) at (#2) {};
%\draw[thick]  ($(#2)+(0.3,-0.01)$) -- ($(#2)+(-0.3,-0.01)$);
%\draw[thick]  ($(#2)+(0.23,0.069)$) -- ($(#2)+(-0.22,0.069)$);
%\draw[thick]  ($(#2)+(0.16,0.139)$) -- ($(#2)+(-0.16,0.139)$);
%\draw[thick]  ($(#2)+(0.09,0.209)$) -- ($(#2)+(-0.09,0.209)$);
%\draw[thick]  ($(#2)+(0.02,0.279)$) -- ($(#2)+(-0.02,0.279)$);
%}
%
%\newcommand{\sground}[2]{
%\node[inner sep=0mm] (#1) at (#2) {};
%\draw[thick]  ($(#2)+(0.2,-0.01)$) -- ($(#2)+(-0.2,-0.01)$);
%\draw[thick]  ($(#2)+(0.12,0.069)$) -- ($(#2)+(-0.12,0.069)$);
%\draw[thick]  ($(#2)+(0.04,0.139)$) -- ($(#2)+(-0.04,0.139)$);
%}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\tikzstyle{every picture}=[baseline=-0.25em]
\tikzstyle{dotpic}=[scale=0.5]
\tikzstyle{diredges}=[every to/.style={diredge}]
\tikzstyle{dot graph}=[shorten <=-0.1mm,shorten >=-0.1mm,scale=0.6]
\tikzstyle{plot point}=[circle,fill=black,minimum width=2mm,inner sep=0]

% create a white box of the given tikz size
\newcommand{\phantombox}[1]{\tikz[baseline=(current bounding box).east]{\path [use as bounding box] (0,0) rectangle #1;}}
\tikzstyle{braceedge}=[decorate,decoration={brace,amplitude=2mm,raise=-1mm}]
\tikzstyle{small braceedge}=[decorate,decoration={brace,amplitude=1mm,raise=-1mm}]
\tikzstyle{left hook arrow}=[left hook-latex]
\tikzstyle{right hook arrow}=[right hook-latex]

\newcommand{\measurement}{\tikz[scale=0.6]{ \draw [use as bounding box,draw=none] (0,-0.1) rectangle (1,0.7); \draw [fill=white] (1,0) arc (0:180:5mm); \draw (0,0) -- (1,0) (0.5,0) -- +(60:7mm);}}

% ================
% = GHZ/W STYLES =
% ================

\tikzstyle{black dot}=[inner sep=0.7mm,minimum width=0pt,minimum height=0pt,fill=black,draw=black,shape=circle]

% TODO: phase out 'dot'
\tikzstyle{dot}=[black dot]
\tikzstyle{smalldot}=[inner sep=0.4mm,minimum width=0pt,minimum height=0pt,fill=black,draw=black,shape=circle]%NEW
\tikzstyle{white dot}=[dot,fill=white]
\tikzstyle{antipode}=[white dot,inner sep=0.3mm,font=\footnotesize]
\tikzstyle{smallwhitedot}=[smalldot,fill=white]%NEW
\tikzstyle{alt white dot}=[white dot,label={[xshift=3.07mm,yshift=-0.05mm,font=\footnotesize]left:$*$}]
\tikzstyle{gray dot}=[dot,fill=gray!40!white]
\tikzstyle{smallgraydot}=[smalldot,fill=gray!40!white]%NEW
\tikzstyle{box vertex}=[draw=black,rectangle]
\tikzstyle{small box}=[box vertex,fill=white]%% added rwd]
\tikzstyle{whitebg}=[fill=white,inner sep=2pt]
\tikzstyle{graph state vertex}=[sg vertex,fill=black]

\tikzstyle{wide copoint}=[fill=white,draw=black,shape=isosceles triangle,shape border rotate=90,isosceles triangle stretches=true,inner sep=1pt,minimum width=1.5cm,minimum height=5mm]
\tikzstyle{wide point}=[fill=white,draw=black,shape=isosceles triangle,shape border rotate=-90,isosceles triangle stretches=true,inner sep=1pt,minimum width=1.5cm,minimum height=4mm]
\tikzstyle{very wide copoint}=[fill=white,draw=black,shape=isosceles triangle,shape border rotate=-90,isosceles triangle stretches=true,inner sep=1pt,minimum width=2.5cm,minimum height=4mm]
\tikzstyle{very wide empty copoint}=[draw=black,shape=isosceles triangle,shape border rotate=-90,isosceles triangle stretches=true,inner sep=1pt,minimum width=2.5cm,minimum height=4mm]
\tikzstyle{symm}=[ultra thick,shorten <=-1mm,shorten >=-1mm]

% ====================================
% = GENERAL MONOIDAL CATEGORY STYLES =
% ====================================

\tikzstyle{square box}=[rectangle,fill=white,draw=black,minimum height=5mm,minimum width=5mm,font=\small]
\tikzstyle{square gray box}=[rectangle,fill=gray!30,draw=black,minimum height=6mm,minimum width=6mm]
\tikzstyle{copoint}=[regular polygon,regular polygon sides=3,draw=black,scale=0.75,inner sep=-0.5pt,minimum width=7mm,fill=white]
\tikzstyle{point}=[regular polygon,regular polygon sides=3,draw=black,scale=0.75,inner sep=-0.5pt,minimum width=7mm,fill=white,regular polygon rotate=180]
\tikzstyle{gray point}=[point,fill=gray!40!white]
\tikzstyle{gray copoint}=[copoint,fill=gray!40!white]

\newcommand{\edgearrow}{{\arrow[black]{>}}}
\newcommand{\edgetick}{{\arrow[black,scale=0.7,very thick]{|}}}
% \pgfkeys{/tikz/.cd, markat/.store in=\markat, markwith/.store
% in=\markwithsym}

% \tikzstyle{diredge}=[postaction=decorate,decoration={markings, mark=at position 0.55 with \edgearrow}]
% \tikzstyle{medium diredge}=[postaction=decorate,decoration={markings, mark=at position 0.75 with \edgearrow}]


\tikzstyle{diredge}=[->]
\tikzstyle{rdiredge}=[<-]
\tikzstyle{medium diredge}=[->]



\tikzstyle{short diredge}=[->]
\tikzstyle{halfedge}=[-)]
\tikzstyle{other halfedge}=[(-]
\tikzstyle{freeedge}=[(-)]
\tikzstyle{white edge}=[line width=5pt,white]
\tikzstyle{tick}=[postaction=decorate,decoration={markings, mark=at position 0.5 with \edgetick}]
\tikzstyle{small map edge}=[|-latex, gray!60!blue, shorten <=0.9mm, shorten >=0.5mm]
\tikzstyle{thick dashed edge}=[very thick,dashed,gray!40]
\tikzstyle{map edge}=[|-latex,very thick, gray!40, shorten <=1mm, shorten >=0.5mm]
\tikzstyle{tickedge}=[postaction=decorate,
  decoration={markings, mark=at position 0.5 with \edgetick}]
% \tikzstyle{dirtickedge}=[postaction=decorate,
%   decoration={markings, mark=at position 0.3 with \edgearrow},
%   decoration={markings, mark=at position 0.5 with \edgetick},
%   decoration={markings, mark=at position 0.8 with \edgearrow}]
\tikzstyle{dirtickedge}=[postaction=decorate,
  decoration={markings, mark=at position 0.5 with \edgetick},
  decoration={markings, mark=at position 0.85 with \edgearrow}]
\tikzstyle{dirdoubletickedge}=[postaction=decorate,
  decoration={markings, mark=at position 0.4 with \edgetick},
  decoration={markings, mark=at position 0.6 with \edgetick},
  decoration={markings, mark=at position 0.85 with \edgearrow}]

% PARALLELAGRAM BOXES:
\makeatletter
\newcommand{\boxshape}[3]{%
\pgfdeclareshape{#1}{
\inheritsavedanchors[from=rectangle] % this is nearly a rectangle
\inheritanchorborder[from=rectangle]
\inheritanchor[from=rectangle]{center}
\inheritanchor[from=rectangle]{north}
\inheritanchor[from=rectangle]{south}
\inheritanchor[from=rectangle]{west}
\inheritanchor[from=rectangle]{east}
% ... and possibly more
\backgroundpath{% this is new
% store lower right in xa/ya and upper right in xb/yb
\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y

\@tempdima=#2
\@tempdimb=#3

\pgfpathmoveto{\pgfpoint{\pgf@xa - 5pt + \@tempdima}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa - 5pt - \@tempdima}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb + 5pt + \@tempdimb}{\pgf@yb}}
\pgfpathlineto{\pgfpoint{\pgf@xb + 5pt - \@tempdimb}{\pgf@ya}}
\pgfpathlineto{\pgfpoint{\pgf@xa - 5pt + \@tempdima}{\pgf@ya}}
\pgfpathclose
}
}}


\boxshape{NEbox}{0pt}{8pt}
\boxshape{SEbox}{0pt}{-8pt}
\boxshape{NWbox}{8pt}{0pt}
\boxshape{SWbox}{-8pt}{0pt}
\makeatother

\tikzstyle{map}=[draw,shape=NEbox,inner sep=7pt]
\tikzstyle{mapdag}=[draw,shape=SEbox,inner sep=7pt]
\tikzstyle{maptrans}=[draw,shape=SWbox,inner sep=7pt]
\tikzstyle{mapconj}=[draw,shape=NWbox,inner sep=7pt]



% PROBABILITY DISTRIBUTION
\tikzstyle{probs}=[shape=semicircle,fill=gray!40!white,draw=black,shape border rotate=180,minimum width=1.2cm]

% ========================
% = COMMUTATIVE DIAGRAMS =
% ========================

\tikzstyle{arrs}=[-latex,font=\small,auto]
\tikzstyle{arrow plain}=[arrs]
\tikzstyle{arrow dashed}=[dashed,arrs]
\tikzstyle{arrow bold}=[very thick,arrs]
\tikzstyle{arrow hide}=[draw=white!0,-]
\tikzstyle{arrow reverse}=[latex-]
\tikzstyle{cdnode}=[]

% =================================
% = Qutrit trichromatic calculus =
% =================================

\tikzstyle{gn}=[dot,fill=lime!50,minimum width=0.2cm,inner sep=0.5pt,font=\footnotesize]
\tikzstyle{rn}=[dot,fill=red!50,inner sep=0.5pt,minimum width=0.2cm,font=\footnotesize]
\tikzstyle{bn}=[dot,fill=blue,minimum width=0.3cm]

\tikzstyle{rc}=[dot,thick,fill=white,draw = red,minimum width=0.2cm,inner sep=0.5pt,font=\footnotesize]
\tikzstyle{gc}=[dot,thick,fill=white,draw= lime,inner sep=0.5pt,minimum width=0.2cm,font=\footnotesize]
\tikzstyle{bc}=[dot,thick,fill=white,draw= blue,minimum width=0.3cm]

\tikzstyle{label}=[circle,fill=white,minimum width=0.3cm]

%\tikzstyle{H box}=[rectangle,draw=black,xscale=1,yscale=1,font=\small,inner sep=0.75pt]
\tikzstyle{H box}=[rectangle,fill=yellow,draw=black,xscale=1,yscale=1,font=\small,inner sep=0.75pt,minimum width=0.15cm,minimum height=0.15cm]

\tikzstyle{clocklabel}=[dot,fill=yellow,draw=black,font=\tiny,inner sep=0.75pt]


\tikzstyle{rsn}=[circle split,draw,fill=red,font=\tiny,inner sep=0.75pt]
\tikzstyle{gsn}=[circle split,draw,fill=lime,font=\tiny,inner sep=0.75pt]
\tikzstyle{bsn}=[circle split,draw,fill=blue,font=\tiny,inner sep=0.75pt]

\tikzstyle{rsc}=[circle split,thick,draw= red,draw,fill=white,font=\tiny,inner sep=0.75pt]
\tikzstyle{gsc}=[circle split,thick,draw= lime,draw,fill=white,font=\tiny,inner sep=0.75pt]
\tikzstyle{bsc}=[circle split,thick,draw= blue,draw,fill=white,font=\tiny,inner sep=0.75pt]

% ========
% = MISC =
% ========

\tikzstyle{cnot}=[fill=white,shape=circle,inner sep=-1.4pt]
% \tikzstyle{tick}=[sloped,rotate=90,font=\small\bf,xshift=0.07mm]
\tikzstyle{wire label}=[font=\tiny, auto]





==> dedication.tex <==
\begin{dedication}
This thesis is dedicated to\\
 someone\\
for some special reason\\
\end{dedication}
